Heron-Bench: A Benchmark for Evaluating Vision Language Models in Japanese

Vision Language Models (VLMs) have undergone a rapid evolution, giving rise to significant advancements in the realm of multimodal understanding tasks. However, the majority of these models are trained and evaluated on English-centric datasets, leaving a gap in the development and evaluation of VLMs for other languages, such as Japanese. This gap can be attributed to the lack of methodologies for constructing VLMs and the absence of benchmarks to accurately measure their performance. To address this issue, we introduce a novel benchmark, Japanese Heron-Bench, for evaluating Japanese capabilities of VLMs. The Japanese Heron-Bench consists of a variety of imagequestion answer pairs tailored to the Japanese context. Additionally, we present a baseline Japanese VLM that has been trained with Japanese visual instruction tuning datasets. Our Heron-Bench reveals the strengths and limitations of the proposed VLM across various ability dimensions. Furthermore, we clarify the capability gap between strong closed models like GPT-4V and the baseline model, providing valuable insights for future research in this domain. We release the benchmark dataset and training code to facilitate further developments in Japanese VLM research.

==> template <==
以下の英語の文章を元の日本語の文章を参考に修正してください。単純な日本語訳ではなく、日本語の文章の意味を理解し、英語の文章を修正してください。

##Part

Methodology


##Original Japanese text

```latex

モデルの評価に関しては, 提案手法であるHeron-benchに加えてLLaVA-Bench (COCO)とLLaVA-Bench (In-the-wild)をDeepLを用いて日本語訳し, 手動で微修正した評価セットも使用する. 
オンラインで利用可能なオープンなVLMに加えて, API経由でアクセスできるクローズドなVLMについても評価を行った. 本論文で構築したVLMに加えて評価対象にしたモデルは以下のとおりである. 

\begin{enumerate}
  \item[Closed: ] GPT-4V, Claude 3 Opus, Gemini Pro Vision
  \item[Open: ] Heron-BLIP v1, Heron-GIT, LLaVA-1.6\footnote{https://huggingface.co/liuhaotian/llava-v1.6-vicuna-7b}, \\LLaVA-1.5\footnote{https://huggingface.co/liuhaotian/llava-v1.5-7b}, Qwen-VL\footnote{https://huggingface.co/Qwen/Qwen-VL}, Japanese Stable VLM\footnote{https://huggingface.co/stabilityai/japanese-stable-vlm}
\end{enumerate}


```


##Target English text

```latex

\subsection{Vision Language Models}

We evaluate six representative vision-language models on Heron-Bench:
Heron-BLIP v1: A model that combines a vision encoder and a language model for multimodal understanding.
Heron-GIT: A generative image-to-text transformer for vision and language tasks.
LLaVA: A large language and vision assistant that connects a vision encoder with a large language model.
GPT-4V: A multimodal variant of GPT-4 that incorporates visual information.
Claude 3 Opus: A multimodal AI assistant that combines visual and language understanding.
Qwen-VL: A vision-language model that employs a query-based attention mechanism.
These models cover a range of architectures and training strategies, providing a comprehensive assessment of the current state-of-the-art in vision-language modeling.

\subsection{Experimental Setup}

We evaluate the six VLMs on Heron-Bench using the proposed circular evaluation strategy. Each model is asked to answer the multiple-choice questions in the dev and test sets. For each question, the model is presented with the image, question, and choices, and is required to select the correct answer. The circular evaluation strategy rotates the choices multiple times, and the model must consistently provide the correct answer to be considered successful.


```


==> template2 <==
You are a professional scientist and have excellent skills of writing a good science paper in deep learning
以下の日本語の文章を英語にしてください。単純な日本語訳ではなく、日本語の文章の意味を理解し、英語の文章を作成してください。複雑な表現は使わない。文章を長くしすぎない。ストレートでわかりやすい表現をする。曖昧な表現をしない。

##Part

Experiment


##Original Japanese text

```latex


\subsubsection{定性評価}
Heron-Benchのスコアと具体的な回答例を基に定性評価を行う. 表2から表4に, Heron-Benchの質問に対するモデルの回答例を示す.

表2に示す単純な会話形式の質問に関しては, Heron GITはGPT-4VやClaude 3 Opusと同等の回答能力を示した. 実験対象のオープンモデルの中で, Heron GITは特に会話 (Conversation) カテゴリーにおいて最も高いスコアであり, これは人間による主観的評価とも一致していた.

表3には, 横綱の土俵入りの写真に対する説明を求める質問とその回答を示す. 全てのモデルが誤った回答をしていた. 特筆すべきは, 写真には3人の力士が映っているにも関わらず「2人の力士が対戦している」のような回答が多かったことである. これは, 相撲が通常2人で行われるという一般的な知識に影響された結果と考えられる. このような日本特有の文化や知識を問う質問に対して, クローズドモデルも不正確な回答をしている事例が複数確認できた. このことから, Heron-Benchは日本固有の知識を問うVQAにおいて有効なベンチマークであることが示唆される.

表4の質問に対する回答では, Heron GIT, GPT-4V, Claude 3 Opusのいずれも赤信号を認識し, 停止の判断をしている. 一方で, 信号機と交通作業員の指示の両方を正しく理解できていたのは, GPT-4Vのみであった. このように, コンテキストの詳細な理解が求められる質問や, 重要な視覚情報が含まれる場合において, GPT-4Vは特に正しい回答をしていた. Heron-Benchは, これらの違いをスコアに適切に反映できていると考えられる. 



```

